On the Regularity of Attention

Attention is a powerful component of modern neural networks across a wide variety of domains. In this paper, we seek to quantify the regularity (i.e. the amount of smoothness) of the attention operation. To accomplish this goal, we propose a new mathematical framework that uses measure theory and integral operators to model attention. We show that this framework is consistent with the usual definition, and that it captures the essential properties of attention. Then we use this framework to prove that, on compact domains, the attention operation is Lipschitz continuous and provide an estimate of its Lipschitz constant. Additionally, by focusing on a specific type of attention, we extend these Lipschitz continuity results to non-compact domains. We also discuss the effects regularity can have on NLP models, and applications to invertible and infinitely-deep networks.

==> main_analysis.tex <==
\section{Structural Analysis of Attention}\label{sec:analysis}

We have proposed a model of attention that encompasses transformers and is amenable to mathematical analysis. 
%In the following sections, 
We will now exploit the model using tools from analysis on the space $\calP(E)$ to study attention in various contexts. %These analyses yield conceptual %insights about how and why %self-attention works. 
We first seek to understand ways in which $\Psi_G$ and $\Pi$ implement a feature extractor from a collection of inputs $\mbf{x}=\{x_1,\dots,x_T\}$ (the deterministic lookup-table implementation of the lookup kernel is not relevant to this analysis, WLOG assume it is the identity).


The {\bf 1-Wasserstein distance} between $\mu,\nu\in \calP_1(E)$ is 
\[
	\W_1(\mu,\nu):=\inf_{\pi\in \calC(\mu,\nu)} \iint_{E\times E}\|x - y\|_1 \pi(\dd x, \dd y)
\] where $\calC(\mu,\nu)$ is the set of distributions on $(E\times E,\calE\times\calE)$ with marginals $\mu,\nu$ on the first and second components, respectively. $\W_1$ is a metric on $\calP_1(E)$ which turns the pair $\calW_1:=(\calP_1(E),\W_1)$ into a complete, separable metric space \cite[ Ch 6]{villani2008optimal} called the \textbf{1-Wasserstein space}. We equip $\calW_1$ with the Borel $\sigma$-algebra induced by $\W_1$. \nnewline

We will also need the generalized entropy functional: let $\nu\in \calP(E)$ and define $H_\nu:\calP(E)\to \R\cup\{\infty\}$ by
\[
	H_\nu(\mu) := \rl{
		-\KL(\mu\|\nu)& \text{ if }\mu\ll \nu\\
		\infty & \text{ otherwise}.
	}
\]
where $\KL(\mu\|\nu) := \int \log\left(\diff{\mu}{\nu}\right) \dd \nu$ denotes the Kullback-Leibler divergence. This cost functional on $\calP(E)$ generalizes the entropy functional to non-uniform base measures.

\begin{definition}[Measure Convolution]
	Let $\mu,\nu\in \calP(\R^d)$ be measures. Then we define the \defn{measure convolution} of $\mu$ and $\nu$, denoted $\mu*\nu$, by
	\[
		(\mu*\nu)(f) := \int f(x+y)\mu(\dd x)\nu(\dd y)~~~\forall f\in \calB_b(\R^d)
	\]
	where $\calB_b(\R^d)$ denotes the space of bounded, measurable functions from $\R^d$ to $\R$.
	\end{definition}


\subsection{The Boltzmann-Gibbs Transformation $\Psi_G$}

Recall that a collection of inputs $X=\{\delta_{x_1},\dots,\delta_{x_N}\}$ has joint configuration $m(X)$, and that the attention kernel $\mbf{A}$ produces new representations $\delta_{x_i}\mbf{A}_{m(X)}$ and a new joint configuration  $m(X)\mbf{A}_{m(X)}$ by nonlinear Markov transport\footnote{By nonlinear Markov transport, we mean that the mass of a measure $\mu$ is transported by a Markov kernel $\mbf{A}$ which \emph{depends on the measure} $\mu$, i.e. $\mu\mapsto \mu\mbf{A}_\mu$}. These new measures have encoded in them features about the inputs; our goal is to understand this process.\nnewline

Recall from Section~\ref{sub:features} that we say a measure $\mu\in \calP(E)$ encodes a feature $f\in E'$ w.r.t. a function $F:E\to E'$ if $\mu(F)=f$. Self-attention has the ability to extract features that depend on the inputs --- this was the original motivation for the attention mechanism in \cite{bahdanau2014neural}. Therefore we replace the function $F$ from above with a bi-measurable map $k:E\times E\to E'$ so that for any fixed $x\in E$,  $\mu$ encodes a feature $f(x)\in E'$ w.r.t. $k(x,\bdot)$, i.e. $\mu(k(x,\bdot))=f(x)$.\nnewline

Suppose now that $m(X)$ and $x$ are fixed, and that $\Psi_{G(x,\bdot)}(m(X))$ encodes $f(x)$ w.r.t. $k(x,\bdot)$. Then we will show that the measure $\Psi_{G(x,\bdot)}(m(X))$ is actually optimal among \emph{all} measures $\mu_x\ll m(X)$ which encode $f(x)$ w.r.t. $k(x,\bdot)$ in the maximum entropy sense. This property characterizes the Softmatch kernel. \nnewline

In this section and the next, we make the assumption below, which will hold unless otherwise stated.
% \vspace{-0.3cm}
\begin{assumption}\label{assump:1}
	$E\subset\R^d$ is a compact, convex set\footnote{Convexity is assumed only to guarantee that the moment-projection onto $\calP_\delta(E)$ is well-defined.}.
\end{assumption}

\begin{restatable}{theorem}{maxent}\label{thm:maxent}
	Let $k:E\times E\to E'$ be a bi-measurable bounded function, $f:E\to E'$ a measurable function, and $\nu\in \calW_1$ be fixed. Define the set
	\[
		\calQ(\nu,x):=\{\mu\in \calW_1\st \mu\ll \nu,~~~\mu(k(x,\bdot)) = f(x)\}, ~\forall x\in E.
	\] Then for each $x\in E$, there exists a unique maximizer $\mu^*_x$ to the maximum entropy problem
	\begin{equation}\label{eq:maxent}
		\max_{\mu_x\in \calQ(\nu,x)} H_\nu(\mu_x)
	\end{equation}
	given by $\mu^*_x=\Psi_{G(x,\bdot)}(\nu)$ with $G(x,y)=\exp\ip{\lambda(x)}{k(x,y)}$ for some $\lambda(x)\in \R^{d'}$. Furthermore, $x\mapsto \mu^*_x$ is measurable, so $(x,\dd y)\mapsto \mu^*_x(\dd y)$ is the Markov kernel $(x,\dd y)\mapsto\Psi_{G(x,\bdot)}(\nu)(dy)$.
\end{restatable}
% $(x,B)\mapsto \Psi_{G(x,\bdot)}(\nu)(B)~\forall x,B\in E\times \calE$.

%\james{The proof sketches (everywhere) need to be updated}
\begin{proof}[Proof Sketch]
	See Appendix~\ref{proof:maxent} for the full proof. Existence and uniqueness of $\mu^*_x$ are classical results. To ensure that $\mu^*_x$ coincides with the Markov kernel $\Psi_{G(x,\bdot)}(\nu)$ we use the additional result that $x\mapsto \mu^*_x$ is measurable which is a technical measurable selection theorem in the appendix. 
\end{proof}

The maxent property is not particularly surprising, given the well-known properties of the softmax and maximum entropy, but it is not \emph{a priori} clear that the dependence of such a measure on $x$ should posess any good properties. We show that the pointwise maximum entropy measure depends measurably on $x$ if $k,f$ are measurable, so the former is indeed the the softmatch kernel\footnote{This is actually a stronger result --- to be a Markov kernel, we need $x\mapsto \mu^*_x(A)$ to be measurable for each $A\in \calE$, but we have actually shown that $x\mapsto \mu^*_x$ as a mapping from $E\to \calP(E)$ is measurable.}.

\begin{remark}
	The minimization problem \eqref{eq:maxent} is an instance of the ``information projection'' operator \citep{koller2009probabilistic}. Below, we see how it relates to the dual notion of moment projection.
\end{remark}

\subsection{The Moment Projection $\Pi$}
Without the moment projection $\Pi$ in the definition of the attention kernel $\mbf{A}$, successive applications of $\mbf{A}$ would result in a measure of arbitrary complexity. On the other hand, we work with finite-dimensional representations, so using the entire space $\calP(E)$ is simply too large to be practical. Therefore, we view $\Pi_\calF:\calP(E)\to \calF$ as a crucial element of attention which ensures that the output measure remains on a finite-dimensional subspace of $\calP(E)$ while preserving moments.\nnewline % encoded therein.

We study two choices of $(\calF,F)$. The first is when $\calF$ is an exponential family on $E$ with sufficient statistics $F$ and base measure $\lambda$, $\calF:=\left\{\nu_\theta(\dd x ) = e^{\ip{\theta}{F(x)} - A(\theta)}\lambda(\dd x) \st \theta\in \R^{d'}\right\}$ and the second is $\calF = \calP_\delta(E)$ with $F(x)=x$. Our main result in this section is a connection between the ``synthetic'' definition of $\Pi$ with an ``analytic'' description as a minimization problem.

\begin{restatable}{proposition}{expmomproj}\label{prop:expmomproj}
	Let $E \subseteq\R^d$ and $\calF$ be a natural exponential family with sufficient statistics $F:E\to E'\subseteq\R^{l}$ and base measure $\lambda$ supported on $E$ as above. Suppose that, for $\mu\in \calP(E)$, $\mu\sim \nu,~\forall \nu\in \calF$. Then $\Pi:\calP(E)\to \calF$ satisfies the projection-like equation
	\[
		\Pi(\mu) = \arg\min_{\nu \in \calF}\KL(\mu\|\nu).
	\]
\end{restatable}

See Appendix~\ref{proof:expmomproj} for the proof, which is standard. Extending the result to the case of $\calF=\calP_\delta(E)$ and $F(x)=x$ requires different arguments because $\mu\not\ll\nu$ in general. Intuitively, we can think of $\calP_\delta(E)$ as a the limit of exponential family $\calF_\sigma:=\{\calN(\dd x,\sigma)\st x\in E\}$ as $\sigma\to 0$. Our approach leverages properties of $F$ and convolution with $\calN(\dd x,\sigma)$ to regularize $\calF$ and $\Pi$ while preserving the encoded moments, then take a limit as $\sigma\to 0$.

\begin{restatable}{proposition}{deltamomproj}\label{prop:deltamomproj}
	Let $\mu\in \calW_1$, and $F(x) = x$. Setting $\calF_n :=   
	\{\rho_n * \delta_x\st \delta_x\in \calP_\delta(E)\}$ $(= \{\calN(x,\sigma_n I), x\in E\})$, where 
	$\rho_n:=\calN(0,\sigma_n I)$ 
	with $\sigma_n\to 0$, then in the 1-Wasserstein topology:
	\[
		\Pi_\calF(\mu) = \lim_{n\to \infty}\arg\min_{\nu\in \calF_n}\KL(\rho_n*\mu\|\nu).
	\]
\end{restatable}

\begin{proof}[Sketch]
    The idea of the proof is to regularize both $\mu$ and $\calF$ by convolution with a sequence of Gaussians $\rho_n$, thereby ensuring that $\rho_n*\mu$ and $\nu\in \calF_n$ have the same supports without affecting the encoded moments.  Theorem~\ref{prop:expmomproj} then applies, and the we show that the sequence of regularized minimizers tends to $\Pi_\calF(\mu)$.
\end{proof}
\begin{remark}
	On a practical note, the choice of $\calF$ can greatly affect how efficient $\Pi$ is to compute. When $\calF = P_\delta(E)$ and $F(x)=x$, then this reduces to linear algebra operations since elements of $\calP_\delta(E)$ (and mixtures thereof) have easy closed-form moments. On the other hand, if $\calF$ is an arbitrary exponential family, e.g. Gaussians with $F(x)=[x\|x^2]$, then a closed form solution to $\mu(F)$ or $\Psi_{G}(\mu)$ may not exist, so one is reduced to computing the projection and/or the normalizing constant via approximation.
\end{remark}

\subsection{Interaction Between the Components}
	We have seen how the transformation $\Psi_G$ extracts a set of features determined by $G$ and encodes them as moments into $\mu=\Psi_G(\nu)$ in a maximum-entropy transformation. The cost to pay for this encoding is an expansion of the degrees of freedom of the measure, i.e. $\mu$ no longer lives in the finite-dimensional moment subspace $\calF_F$. On the other hand, the projection $\Pi$ ``squeezes'' the measure $\mu$ through a bottleneck, reducing the degrees of freedom to those determined by $\calF_F$. This is a accomplished via the moment projection, and can be seen as discarding extra information in the system while preserving a set of moments determined by $F$. 

==> main_structured.tex <==
\section{Structured Data, and Random Fields, and Measures}
\remi{Wondering whether this section should be merged with Notations and preliminaries}
\aristide{In fact I would even move the current Sec 1.1 to the Appendix (and/or release the defs on the fly in text) and replace it by this Section 3}\remi{I'm fine with the Markov kernel part of the notations. Agreed about the more mainstream definitions like TV and KL}\james{Make a precise definition of structured data}
In this section, we consider the problem of unifying the treatment of ``structured data'' by an attention based model. We consider structured data to be collections of distinct elements together with some structure describing their relationships. Text, graphs, and images all fit neatly within this very broad description, and our first task is to show how these three modalities are instances of random fields. Then we will show how to associate to these structured data a measure, and how ``features'' of these data are represented.

\subsection{Structured Data}
\james{Structured data is any data which can be modelled by a random field.}
\begin{definition}[Random Field]
	Let $(\Omega,\calF,\P)$ be a probability space. Let $\calT$ be a topological space. Let $(S,\calS)$ be a measurable state space. A random field $\mbf{x}$ is a collection of random variables on $\Omega$ indexed by $\calT$, i.e. $\mbf{x}=\{x_t\}_{t\in \calT}$ where $x_t:\Omega\to S$.
\end{definition}
In this paper, we will assume that $\calT$ and $S$ are discrete, finite sets. For statistical modelling, we are interested in approximating the law of $\mbf{x}$, denoted $P:=\mbf{x}_*\P$, by another measure $Q$. Moreover, we will assume the existence of a neighbourhood mapping $\calN:\calT\to 2^\calT$ such that
\[
	P(x_t|\mbf{x}_{-t}) = P(x_t | \calN(t)).
\]where we have used $-t:=\calT\setminus\{t\}$. In general, this imposes no restrictions on $P$ since $\calN(t)$ can be arbitrary and it is a result due to \cite{besag1974spatial} that knowledge of the complete conditionals is sufficient to uniquely determine the joint law. On the other hand, statistical modelling text, graphs, and images are instances of modelling such a law, therefore we will consider random field modelling in the remainder of this paper.

\subsection{Measures \& Features}
\label{sub:features}
The nature of self-attention, as we will see below, is best\james{don't use superlatives w/o justification} modelled as a measure-transport phenomenon. Therefore, in preparation for this, we establish some key concepts.

Firstly, we define the empirical measure mapping. Let $E\in \calB(\R^d)$ be a Borel-measurable subset. There is a natural bijection between $E$ and $\calP_\delta(E):=\{\delta_x\st x\in E\}$ induced by the mapping
\[
	x\mapsto \delta_x.
\]This way, we can associate any random field with state space $S\subset E$ to a measure in $\calP(E)$:
\[
	\mbf{x}\mapsto m(\mbf{x}):=\frac{1}{|\calT|}\sum_{t\in \calT} \delta_{x_t}.
\]{\todo this mapping is not exchangeable} This mapping appears to be the ``right'' setting for studying the action of self-attention.\remi{Justify, or say something like: As we will see later, this setting allows us to model self-attention as an object acting on measures amenable to self-composition blabla.} We also define the inverse mapping on the set of uniform empirical measure: $m^{-1}(\frac{1}{|\calT|}\sum_{t\in \calT} \delta_{x_t}) = (x_t)_{t \in \calT}$.


Secondly, we establish the concept of a feature encoded in a measure\remi{Is this a classic way of doing things? If so, reference?}. Let $F:E\to E'\subset \R^{d'}$ be a measurable map, representing a feature extractor \james{terrible terminology}. We say that a measure $\mu\in \calP(E)$ encodes features $f\in E'$ w.r.t. $F$ if $\mu(F)=f$. This notion is particularly useful when $E'=E$ and $F(x)=x$ in which case $\delta_x(F)=x$, and $\delta_x$ encodes feature $x$. This will allow us to translate notions about vector-space representations to notions about measures and the features they encode.

Moreover, we can parameterize families of measures by the features they encode. Let \mbox{$F:E\to E'$} be fixed, and suppose we have identified a mapping $f\mapsto \nu_f\in \calP(E)$ which is a bijection \aristide{ injection, no?} and for which $\nu_f(F)=f$. Then we denote by $\calF_F=\{\nu_f\st f\in E'\}$ the family of all such distributions, usually omitting the subscript $F$ when there is no chance of confusion. Two particular cases are a natural exponential family with sufficient statistics $F$, and $\calP_\delta(E)$ for $E'=E$ and $F(x)=x$. We will consider both in the sequel. Finally, we define the feature projection onto $\calF$, denoted $\Pi_\calF:\calP(E)\to \calF$, defined by
\[
	\Pi_\calF(\mu) = \nu_{\mu(F)}.
\]{\todo This mapping will allow us to represent finite-dimensional features with measures while keeping the dimensionality of such representations finite.}
